Implementation feedback of the IVOA Provenance data model

The IVOA Provenance Data model defines entities, agents and activities as container classes to describe the provenance of datasets, with the executed tasks and responsibilities attached to agents. It also provides a set of classes to describe the activities type and their configuration template, as well as the configuration applied effectively during the execution of a task. Here we highlight lessons learned in the implementation of the CDS ProvHiPS service distributing provenance metadata for the HST HiPS data collections, and for the HST archive original images used to produce the HiPS tiles. ProvHiPS is based on the ProvTAP protocol, the emerging TAP standard for distributing provenance metadata. ProvTAP queries may rapidly become very complex. Various graph representation strategies, including ad hoc solutions, triplestore and SQL CTE have been considered and are discussed shortly.

==> Makefile <==
# Example makefile to help you compile your ADASS proceedings
# but you really should read the ManuscriptInstructions.pdf or
# at least the README file. For some smart cookies the Makefile
# could be sufficient too.
#
# Version 27-sep-2019   Peter Teuben
#
# See also:  http://www.adass.org/instructions/ADASS2019.tar
#            https://www.adass2019.nl/proc/ADASS2019.tar
#
# P = paper_id    your proceedings paper ID code (the one with the dash, not dot)
# V = version     your version # (1,2,..) since you can only upload unique files
# A = 1stauthor   your last name, e.g. Teuben
# E = email       your contact email for submission issues
# FIGS = *eps     your EPS figures

                    # put your paper_id here (with dash, not dot), e.g. P10-2
                    # or find your template on http://www.astro.umd.edu/~teuben/adass/papers/
P = P2-6
                    # keep incrementing this after each upload of your $(P)
V = 2
A = Louys           # First author (for Papercheck.py         
E = mireille.louys@unistra.fr     # contact person email
		    # your EPS figures (can be blank, and must be base-named with $(P)_*.eps
FIGS = example.eps

# override P,V,A,E,FIGS with a "makedefs" file, this is where authors should edit, not this Makefile
-include makedefs

#  variables for proceeding editors (don't modify, for export, not for authors)
YEAR   = 2019
TMPDIR = ADASS$(YEAR)_author_template
FILES  = AdassChecks.py AdassConfig.py AdassIndex.py ADASS_template.tex \
	 Aindex.py FixUnprintable.py \
	 asp2014.bst asp2014.sty copyrightform.pdf example.bib example.eps \
	 Index.py manual2010.pdf ManuscriptInstructions.pdf PaperCheck.py \
	 README subjectKeywords.txt TexScanner.py \
	 ascl.py asclKeywords.txt \
	 adass2019.bib Makefile makedefs

#  probably don't change these either (or notify the editors you have a special paper case)
TAR_FILE  = $(P)_v$(V).tar.gz
ZIP_FILE  = $(P)_v$(V).zip
FILES4AR  = $(P).tex $(P).bib $(FIGS) makedefs $(P).pdf copyrightform_$(P)_$(A).pdf

# ensure current directory is in the PATH
export PATH := .:$(PATH)

help:
	@echo AUTHOR targets:
	@echo ---------------
	@echo all:   pdf check tar
	@echo pdf:
	@echo check:
	@echo clean:
	@echo tar:
	@echo zip:
	@echo 
	@echo EDITOR targets:
	@echo ---------------
	@echo fix:
	@echo inc:
	@echo spell:
	@echo aindex:
	@echo words:
	@echo asp1:
	@echo index:   needs TERMS=
	@echo ascl:
	@echo ascl1:
	@echo ascl2:   needs CODE=
	@echo pdf2:
	@echo rsync:


all:	pdf check tar


# not for authors, for creator of the ADASS instruction tar file
export:
	rm -rf $(TMPDIR)
	mkdir $(TMPDIR)
	cp -a $(FILES) $(TMPDIR)
	echo Created on `date` by `whoami`  > $(TMPDIR)/VERSION
	-git remote -v                     >> $(TMPDIR)/VERSION
	-git branch                        >> $(TMPDIR)/VERSION
	tar cf ADASS$(YEAR).tar $(TMPDIR)

# copyright is now part of the tar/zip file, checksum (sum) is 13785
copyrightform_$(P)_$(A).pdf: copyrightform.pdf
	cp copyrightform.pdf copyrightform_$(P)_$(A).pdf
	@echo Now go edit your copyrightform_$(P)_$(A).pdf form

# these targets are for most common unix systems, but YMMV. Modify if you need
# let the editors know you have a better way for the next ADASS team
# ASP prefers the latex;latex;dvipdfm route

DVIPDF = dvipdf

pdf:	$(P).pdf
	@echo xdg-open $(P).pdf 

$(P).pdf:  $(P).dvi $(FIGS)
	$(DVIPDF) $(P)

$(P).bib:                                  # bootstrap if you don't have one
	touch $(P).bib

$(P).dvi:  $(P).tex $(P).bib
	latex $(P)
	if [ -s $(P).bib ]; then bibtex $(P); fi
	latex $(P)
	latex $(P)

# an alternative method (ASP does not recommend it)
pdflatex:
	pdflatex $(P)
	if [ -s $(P).bib ]; then bibtex $(P); fi
	pdflatex $(P)
	pdflatex $(P)

clean:
	rm -f $(P).dvi $(P).bbl $(P).pdf $(P).aux $(P).log $(P).out $(P)_inc.tex

check:
	PaperCheck.py $(P) $(A)

ENCODING =
fix:
	FixUnprintable.py  $(P).tex $(ENCODING)

inc:
	tex2inc.py $(P).tex > $(P)_inc.tex
	@tail -1 $(P)_inc.tex
	@cat $(P).toc

spell:
	aspell --mode=tex check $(P).tex
	@echo Share your ~/.aspell.en.pws  ~/.aspell.en.prepl

aspell:
	(cd ../..; $(MAKE) aspell)

dvi:
	latex $(P)

aindex:
	Aindex.py $(P)

DETEX = detex
words:
	$(DETEX) $(P).tex | grep -o -E '\w+' | tr '[A-Z]' '[a-z]' | sort | uniq -c | sort -n

#  could add a checksum on personal copyrightform - if it's 13785,it's bad.
tar:    $(FILES4AR) _checksum
	tar zcf $(TAR_FILE) $(FILES4AR)
	#@echo Submit to ftp://ftp.astro.umd.edu/incoming/adass
	#@echo e.g.   ncftpput ftp.astro.umd.edu  incoming/adass $(TAR_FILE)

zip:    $(FILES4AR) _checksum
	rm -f $(ZIP_FILE)
	zip $(ZIP_FILE) $(FILES4AR)
	#@echo Submit to ftp://ftp.astro.umd.edu/incoming/adass
	#@echo e.g.   ncftpput ftp.astro.umd.edu  incoming/adass $(ZIP_FILE)

_checksum: copyrightform_$(P)_$(A).pdf
	@echo Checksum test
	@sum copyrightform_$(P)_$(A).pdf

# for editors
asp1:
	(cd ../..; $(MAKE) asp1 PID=$(P); grep box asp1.log)
	@echo xdg-open ../../authors/$(P).pdf

TERMS = foobar
index:
	@echo Using TERMS=$(TERMS)
	(cd ../Author_Template; Index.py $(TERMS))

index2:
	(cd ../adass_subject_recommender ; detex ../$(P)/$(P).tex |  PYTHONPATH=`pwd` bin/find_subjects.py -m 10 -j)

ascl:
	(cd ../Author_Template; ascl.py ../../ADASSProceedings2019/papers/$(P)/$(P).tex)

ascl1:
	(cd ../Author_Template; ascl.py ../../ADASSProceedings2019/papers/$(P)/$(P).tex | grep ooindex | sort | uniq -c)
	-detex $(P).tex > $(P).txt
	-(cd ../Author_Template; ascl.py ../../ADASSProceedings2019/papers/$(P)/$(P).txt | grep ooindex | sort | uniq -c)
	-grep ooindex $(P).tex

CODE = foobar
ascl2:
        xdg-open https://ascl.net/$(CODE)

pdf2:   pdf asp1
	xdg-open $(P).pdf
	xdg-open ../../authors/$(P).pdf

rsync: $(P).bib
	rsync -av $(P)_inc.tex $(P).bib $(FIGS) ../../authors
	rm -f ../../authors/$(P)_inc.{bbl,blg}


